Reading Order Independent Metrics for Information Extraction in Handwritten Documents

Information Extraction processes in handwritten documents tend to rely on obtaining an automatic transcription and performing Named Entity Recognition (NER) over such transcription. For this reason, in publicly available datasets, the performance of the systems is usually evaluated with metrics particular to each dataset. Moreover, most of the metrics employed are sensitive to reading order errors. Therefore, they do not reflect the expected final application of the system and introduce biases in more complex documents. In this paper, we propose and publicly release a set of reading order independent metrics tailored to Information Extraction evaluation in handwritten documents. In our experimentation, we perform an in-depth analysis of the behavior of the metrics to recommend what we consider to be the minimal set of metrics to evaluate a task correctly.

==> Contents/deprecated/ALT_T5-RESULTS.tex <==
%Scores with dd.d format (only 1 decimal)

\begin{table}[htb]
    \centering
    \caption{Comparison between metrics across four datasets. OI refers to Order-Independent metric. The largest 95\% confidence interval computed is $5.6$ for the Nerval-Precision in IAM-18 (regular). Therefore, the OI version of the text-alignment metrics obtains a statistically significant difference compared to their original version. }
    \label{tab:table5-1}
    \begin{tabular}{l|cc|cc|cc|cc}
        \toprule
     %   \rule{0pt}{4ex}  \multirow{3}{*}{\textbf{Metrics}} & \multicolumn{8}{c}{\textbf{Dataset}} \\
        
        & \multicolumn{2}{c|}{\textbf{IAM-18}} & \multicolumn{2}{c|}{\textbf{Simara}} & \multicolumn{2}{c|}{\textbf{Esposalles}} & \multicolumn{2}{c}{\textbf{POPP}} \\ 
        \textbf{Dataset}  & regular & shuffled & regular & shuffled & regular & shuffled & regular & shuffled \\
        \midrule
        CER $\downarrow$ & 5.0 & 74.2 & 6.4 & 39.7 & 0.4 & 68.1 & 8.8 & 67.5 \\
        WER $\downarrow$ & 15.5 & 94.0 & 17.3 & 54.2 & 1.5 & 84.2 & 23.6 & 80.5 \vspace{0.4em}\\ 
        
        ECER $\downarrow$ &  86.5 &  98.2 & 5.0 & 74.0 & 3.6 & 88.5 & 9.2 & 79.2 \\
        OIECER $\downarrow$ &  83.7 &  83.7 & 5.0 & 5.0  & 3.5 &  3.5 &  9.2 & 9.2  \vspace{0.4em}\\
        
        EWER $\downarrow$ &  93.3 &  103.3 & 10.2 & 75.5 & 4.8 & 88.8 & 20.9 & 82.4 \\
        OIEWER $\downarrow$ &  91.5 &  91.5 & 10.2 & 10.2 &  4.7 & 4.7 & 20.9 & 20.9 \vspace{0.4em}\\
        
        Nerval-Precision $\uparrow$ & 29.0 & 2.9 & 95.0 & 37.7 & 96.3 & 17.0 & 89.3 & 35.0 \\
        OINerval-Precision $\uparrow$ & 29.0 &  29.0 & 95.0 & 95.0 & 96.3 & 96.3 & 89.3 & 89.3 \vspace{0.4em}\\
        
        Nerval-Recall $\uparrow$ & 26.6 & 2.7 & 95.3 & 37.9 & 97.1 & 17.2 & 90.0 & 35.3 \\
        OINerval-Recall $\uparrow$ &  26.6 &  26.6 & 95.4 & 95.4 & 97.1 & 97.1 & 90.0 & 90.0  \vspace{0.4em}\\
        
        Nerval-F1 $\uparrow$ & 27.7 & 2.8 & 95.1 & 37.8 & 96.7 & 17.1 & 89.6 & 35.1 \\
        OINerval-F1 $\uparrow$ &  27.7 &  27.7 &  95.2 & 95.2 & 96.7 & 96.7 & 89.6 & 89.6 \vspace{0.4em}\\
        
        %BoTWER $\downarrow$ & 100.00 & 100.00 & 31.28 & 31.28 & 7.96 & 7.96 & 44.86 & 44.86 \\ % equation 7
        btWER $\downarrow$ & 85.3 & 85.3 & 17.4 & 17.4 & 4.6 & 4.6 & 24.2 & 24.2  \vspace{0.4em}\\ % equation 8
    
        bt-Precision $\uparrow$ & 29.2 & 29.2 & 84.8 & 84.8 & 95.9  & 95.9 & 77.4 & 77.4 \\
        bt-Recall $\uparrow$ & 21.2 & 21.2 & 83.7 & 83.7 & 96.2 & 96.2 & 78.0 & 78.0 \\ 
        bt-F1 $\uparrow$ & 24.5 & 24.5 & 84.3 & 84.3 & 96.0 & 96.0 & 77.7 & 77.7 \vspace{0.4em}\\
        
        beER $\downarrow$ & 94.2 &  94.2 & 23.2 & 23.2 & 5.8 & 5.8 & 23.1 & 23.1 \vspace{0.4em}\\ %entity based = field-based F1 from donut -> to check
        
        be-Precision $\uparrow$ & 21.6 & 21.6 & 77.1 & 77.1 & 94.4 & 94.4 & 77.4 & 77.4 \\
        be-Recall $\uparrow$ & 19.8 & 19.8 & 77.3 & 77.3 & 95.2 & 95.2 & 78.0 & 78.0 \\ 
        be-F1 $\uparrow$ & 20.7 & 20.7 & 77.2  & 77.2 & 94.8 & 94.8 & 77.7 & 77.7  \vspace{0.4em} \\ %entity based = field-based F1 from donut

   %     TED-Acc $\uparrow$ & 18.7 & 16.0 & 92.7 & 92.7 & 95.7 & 93.6 &  90.3 & 90.3 \\ %TED-acc from donut
        \bottomrule
    \end{tabular}
\end{table}

==> Contents/deprecated/T5-RESULTS.tex <==
%Scores with dd.d format (only 1 decimal)

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{3}{*}{Metrics} & \multicolumn{8}{c|}{Dataset} \\
        \cline{2-9}
        & \multicolumn{2}{c|}{IAM-18} & \multicolumn{2}{c|}{Simara} & \multicolumn{2}{c|}{Esposalles} & \multicolumn{2}{c|}{POPP} \\ 
        & regular & shuffled & regular & shuffled & regular & shuffled & regular & shuffled \\
        \hline
        CER $\downarrow$ & 5.0 & 74.2 & 6.4 & 39.7 & 0.4 & 68.1 & 8.8 & 67.5 \\
        WER $\downarrow$ & 15.5 & 94.0 & 17.3 & 54.2 & 1.5 & 84.2 & 23.6 & 80.5 \\ 
        \hline
        ECER $\downarrow$ &  132.0 &  143.8 & 9.3 & 95.9 & 5.8 & 126.2 & 17.0 &  105.2 \\
        OI-ECER $\downarrow$ &  131.2 &  131.2 & 9.3 & 9.3 & 5.8 & 5.8 & 17.0   & 17.0  \\
        \hline
        EWER $\downarrow$ &  147.0 &  154.4 & 19.6 & 99.7 & 8.3 & 126.9 & 40.5  & 113.6 \\
        OI-EWER $\downarrow$ &  146.8 &  146.8 & 19.6 & 19.6 & 8.3 & 8.3 & 40.5 & 40.5  \\
        \hline
        Nerval-Precision $\uparrow$ & 29.0 & 2.9 & 95.0 & 37.7 & 96.3 & 17.0 & 89.3 & 35.0 \\
        OI-Nerval-Precision $\uparrow$ & 29.0 &  29.0 & 95.0 & 95.0 & 96.3 & 96.3 & 89.3 & 89.3 \\
        \hline
        Nerval-Recall $\uparrow$ & 26.6 & 2.7 & 95.3 & 37.9 & 97.1 & 17.2 & 90.0 & 35.3 \\
        OI-Nerval-Recall $\uparrow$ &  26.6 &  26.6 & 95.4 & 95.4 & 97.1 & 97.1 & 90.0 & 90.0  \\
        \hline
        Nerval-F1 $\uparrow$ & 27.7 & 2.8 & 95.1 & 37.8 & 96.7 & 17.1 & 89.6 & 35.1 \\
        OI-Nerval-F1 $\uparrow$ &  27.7 &  27.7 &  95.2 & 95.2 & 96.7 & 96.7 & 89.6 & 89.6 \\
        \hline
        %BoTWER $\downarrow$ & 100.00 & 100.00 & 31.28 & 31.28 & 7.96 & 7.96 & 44.86 & 44.86 \\ % equation 7
        btWER $\downarrow$ & 85.3 & 85.3 & 17.4 & 17.4 & 4.6 & 4.6 & 24.2 & 24.2 \\ % equation 8
        \hline
        bt-Precision $\uparrow$ & 29.2 & 29.2 & 84.8 & 84.8 & 95.9  & 95.9 & 77.4 & 77.4 \\
        bt-Recall $\uparrow$ & 21.2 & 21.2 & 83.7 & 83.7 & 96.2 & 96.2 & 78.0 & 78.0 \\ 
        bt-F1 $\uparrow$ & 24.5 & 24.5 & 84.3 & 84.3 & 96.0 & 96.0 & 77.7 & 77.7 \\
        \hline
    \end{tabular}
    \caption{Comparison between metrics across the IAM-18, Simara, Esposalles and POPP datasets. Note that OI stands for Order-Independent metric. The largest 95\% confidence interval computed is $6.16$ for the EWER in Simara (shuffled). Therefore, the OI version of the metrics obtain a statistically significant difference compared with their original version. This happens for all the shuffled corpora except in the IAM database for the ECER and EWER metrics. }
    \label{tab:table5-1}
\end{table}
